MLLA-UNet: Mamba-like Linear Attention in an Efficient U-Shape Model for Medical Image Segmentation

Recent advancements in medical imaging have resulted in more complex and diverse images, with challenges such as high anatomical variability, blurred tissue boundaries, low organ contrast, and noise. Traditional segmentation methods struggle to address these challenges, making deep learning approaches, particularly U-shaped architectures, increasingly prominent. However, the quadratic complexity of standard self-attention makes Transformers computationally prohibitive for high-resolution images. To address these challenges, we propose MLLA-UNet (Mamba-Like Linear Attention UNet), a novel architecture that achieves linear computational complexity while maintaining high segmentation accuracy through its innovative combination of linear attention and Mamba-inspired adaptive mechanisms, complemented by an efficient symmetric sampling structure for enhanced feature processing. Our architecture effectively preserves essential spatial features while capturing long-range dependencies at reduced computational complexity. Additionally, we introduce a novel sampling strategy for multi-scale feature fusion. Experiments demonstrate that MLLA-UNet achieves state-of-the-art performance on six challenging datasets with 24 different segmentation tasks, including but not limited to FLARE22, AMOS CT, and ACDC, with an average DSC of 88.32%. These results underscore the superiority of MLLA-UNet over existing methods. Our contributions include the novel 2D segmentation architecture and its empirical validation. The code is available via https://github.com/csyfjiang/MLLA-UNet.

==> sec/intro_draft.tex <==

    

\section{Introduction}
Medical image segmentation is a critical step in computer-aided diagnosis and treatment planning. 
%
With advancements in medical imaging technology, we are confronted with increasingly complex and diverse medical images. 
%
These images often exhibit high anatomical variability, blurred tissue boundaries, low contrast between organs, and imaging noise and artifacts \cite{metheany2008characterizing}. 
%
Traditional segmentation methods often struggle with these complexities, necessitating more advanced techniques to address these challenges effectively~\cite{ma2010review_tm,pham2000current_tm,litjens2017survey_tm,sharma2010automated_tm,vaswani2017attention_transformer}.
%%% End of first paragraph

In recent years, deep learning approaches, particularly models based on convolutional neural networks (CNNs)~\cite{long2015fully_cnn,brosch2016deep_cnn,milletari2016v_cnn,zhou2018unet++_cnn,ronneberger2015u_cnn_unet,badrinarayanan2017segnet_cnn,lecun1998gradient_cnn} and Transformers~\cite{lin2022ds_tran,cao2022swin_tran,tang2022self_tran,chen2021transunet_tran,wu2024medsegdiff_tran_diff,vaswani2017attention_transformer,dosovitskiy2020image_vit}, have made significant progress in medical image segmentation tasks. 
%
However, these methods still face several critical limitations.
%
Traditional self-attention mechanisms have a computational complexity of \(O(n^2)\), making them costly for high-resolution medical images. \textcolor{red}{citation}
%
While Transformers excel at capturing long-range dependencies \textcolor{red}{citation}, they may not preserve local structural information as effectively as CNNs. \textcolor{red}{citation}
%
Additionally, existing models often struggle to adapt to different modalities, such as CT and MRI, and varying anatomical structures. \textcolor{red}{citation}
%
Furthermore, many methods employ complex upsampling strategies, increasing computational overhead and risking overfitting.
%%% End of second paragraph

%SSM在医学分割上的优势,特别的, 看一下相关工作他们为什么使用Mamba为什么不用别的?
%SSM 相较于CNN和Transformer有什么优势(找一下Vision Mamba上说的对自然图像上的分割有什么优点),
% 前人很多用了SSM和U-Shape结合的工作,但是他们有一些问题, 他们的问题是...
%如何体现在医学分割上? 但是Mamba有什么局限性,在previous work (MLLA作者 Han et.al) argue linear attention和mamba是近似,相较于 Vision Mamba有什么其他优势?
% Transformer -> SSM -> MLLA
% MLLA 能解决 SSM/CNN/Transformer的什么问题
To address these challenges, we propose a novel medical image segmentation architecture based on Mamba-Like Linear Attention (MLLA)~\cite{han2024demystify_mlla}.
%
%基于上面的问题,要有一个总结,要有CNN的local-structure的Transformer的long-range Dependency的
% 解决这三个问题的时候的心路历程: 对于这个医学分割的
% 在医学分割上,MLLA带来的independent, 独特的优势在哪? First Second, ....
Our approach offers several key innovations: First, MLLA reduces the computational complexity of the attention mechanism from $O(n^2)$ to $O(n)$~\cite{katharopoulos2020transformers_linearAt}, enabling efficient processing of high-resolution medical images.
% 下面是错的
Second, MLLA's unique state space model allows for adaptive capture of image features at different scales, better handling the diversity of anatomical structures. 
% 对称和不对称的优劣?
Third, our architecture implements symmetric and efficient multi-scale feature fusion through innovative downsampling and simplified upsampling strategies, enhancing the model's ability to segment organs of various sizes and shapes. 
% 是SSM的有点还是MLLA的有点↓
Fourth, the flexible design of MLLA demonstrates excellent cross-modal adaptability, maintaining high performance across different medical imaging modalities. 
%
Finally, we provide an in-depth theoretical analysis explaining why MLLA is particularly well-suited for medical image segmentation tasks, offering new perspectives for future research in this field.
%%%
The main contributions of this paper can be summarized as follows:

\begin{itemize}
    \item We propose a novel medical image segmentation architecture based on MLLA, significantly enhancing segmentation accuracy and computational efficiency.
    % 斟酌一下得益于U-Shape,还是?
    \item We implement a symmetric and efficient sampling structure, incorporating the original MLLA downsampling approach and developing a complementary upsampling method. This unified design optimizes both feature extraction and reconstruction processes, enhancing the overall performance of our segmentation architecture.
    
    \item We demonstrate state-of-the-art (SOTA) performance across multiple challenging medical image datasets, including AMOS22CT/MR~\cite{ji2022amos}, WORD~\cite{luo2021word}, FLARE22~\cite{FLARE22}, ATLAS22~\cite{quinton2023tumour_altas}, BTCV~\cite{btcv}, and ACDC~\cite{acdc}, showcasing the broad applicability of our approach.
    
    \item We offer detailed theoretical analysis and experimental validation, providing in-depth insights into the advantages of MLLA in medical image segmentation. Additionally, we develop a scalable framework that paves the way for new research directions in future medical image analysis tasks.
\end{itemize}


% \usepackage{tabularray}
\begin{table}[H]
\small
\centering
\caption{Ablation study of different configurations of MLLAUNet-T across WORD, FLARE22, AMOSCT, ALTAS22, BTCV, ACDC, and AMOSMR. The ablation focuses on the inclusion of the Stem, Merging, and Expanding components (indicated by \textcolor{green}{\ding{51}} or \textcolor{red}{\ding{55}}). Additionally, the MLLAUNet-T-load-encoder-only row represents a strategy where only the encoder is loaded, while MLLAUNet-Small and MLLAUNet-Base rows represent model variants used to evaluate the impact of model size. The Dice Similarity Coefficient (DSC \%) is used as the evaluation metric, and the average DSC across all datasets is reported in the last column, with the best results highlighted in \textbf{bold} and the second-best results \uline{underlined}.}
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[70]Q[94]Q[100]Q[71]Q[92]Q[96]Q[92]Q[65]Q[67]Q[100]Q[65]},
  cells = {c},
  cell{10}{1} = {c=3}{0.274\linewidth},
  cell{11}{1} = {c=3}{0.274\linewidth},
  cell{12}{1} = {c=3}{0.274\linewidth},
  vline{4,11} = {1-12}{},
  vline{2,11} = {10-12}{},
  hline{1-2,10,13} = {-}{},
}
Stem & Merging & Expanding & WORD & FLARE22 & AMOSCT & ALTAS22 & BTCV & ACDC & AMOSMR & Avg\\
\textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & 80.53 & 85.38 & 82.56 & 73.11 & 78.56 & 84.01 & 78.53 & 80.38\\
\textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & \textcolor{green}{\ding{51}} & 80.12 & 86.54 & 82.38 & 73.36 & 79.6 & 86.34 & 82.22 & 81.51\\
\textcolor{red}{\ding{55}} & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & 79.76 & 84.53 & 80.17 & 72.44 & 78.23 & 84.75 & 80.04 & 79.99\\
\textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & 83.3 & 89.18 & 86.49 & 75.94 & 82.4 & 90.23 & 84.23 & 84.54\\
\textcolor{red}{\ding{55}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & 82.41 & 89.03 & 85.68 & 75.51 & 81.49 & 89.58 & 83.14 & 83.83\\
\textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{green}{\ding{51}} & 84.21 & 90.14 & 86.89 & 78.41 & 82.41 & 90.88 & 85.1 & 85.43\\
\textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & 83.17 & 89.79 & 85.77 & 77.48 & 81.37 & 89.81 & 83.28 & 84.38\\
\textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textbf{89.10} & \textbf{92.76} & \textbf{90.05} & \uline{83.09} & \textbf{85.28} & \textbf{93.28} & \uline{87.29} & \textbf{88.69}\\
LoadEncoderOnly &  &  & \uline{84.82} & 90.1 & \uline{88.51} & 80.19 & 83.21 & 91.05 & 86.25 & 86.3\\
MLLAUNet-Small &  &  & 84.59 & \uline{91.34} & 87.45 & \textbf{84.21} & \uline{83.41} & \uline{91.32} & \textbf{88.33} & \uline{87.24}\\
MLLAUNet-Base &  &  & 83.18 & 90.58 & 86.31 & 79.31 & 82.63 & 90.19 & 85.34 & 85.36
\end{tblr}
\end{table}

% Detailed verision ↓
% At the core of MLLAUNet is the MLLA mechanism, which reduces the computational complexity of the attention mechanism from $O(n^2)$ to $O(n)$~\cite{katharopoulos2020transformers_linearAt}. This reduction in complexity is particularly significant for high-resolution medical images. For instance, consider a typical high-resolution CT scan with dimensions of 512x512 pixels. In a standard attention mechanism, processing this image would require $O((512 \times 512)^2) \approx O(68$ billion$)$ operations. In contrast, our MLLA mechanism reduces this to $O(512 \times 512) \approx O(262$ thousand$)$ operations, a reduction of over five orders of magnitude. This dramatic improvement in computational efficiency enables the processing of high-resolution medical images that would be computationally prohibitive with standard attention mechanisms, while still maintaining the ability to capture long-range dependencies.
%

\subsubsection*{Limitation}
The MLLA-UNet framework represents a significant advancement in medical image segmentation by leveraging model scaling and diverse datasets. However, its effectiveness is limited by challenges specific to medical imaging, such as the significant difference between the features of natural and medical images. This discrepancy makes it difficult for traditional pre-training methods, which use weights from models trained on natural images like ImageNet-1K~\cite{deng2009imagenet}, to be effective in medical contexts. To overcome this, a specialized pre-training regimen for MLLA-UNet needs to be developed~\cite{MIM}, focusing on tasks closely aligned with medical imaging to enhance feature transferability and model robustness. Furthermore, the potential of MLLA-based models for few-shot or zero-shot learning in medical scenarios remains underexplored. Models like the SAM~\cite{SAM} have shown capabilities in similar domains, suggesting that MLLA architectures might also be adapted for effective use with minimal or no labeled data, a significant advantage in settings where annotated medical data is scarce. 
Lastly, the MLLA-UNet framework, which merges the strengths of CNNs, Transformers, and Mamba techniques, offers considerable promise as a foundational model for medical imaging~\cite{FM}. However, there is a significant gap in the thorough theoretical and empirical validation of this innovative approach. To fully realize its potential, extensive research is necessary to evaluate and quantify the benefits of this hybrid model within the medical imaging field. Such studies would focus on examining the adaptability of the MLLA-UNet to various medical imaging tasks and assessing its performance in comparison to more traditional or specialized models. Through detailed evaluation and validation, the capabilities of the MLLA-UNet can be enhanced, further contributing to the broader field of medical image analysis by offering a more adaptable and robust toolset suitable for the diverse and complex datasets typically found in medical contexts.
